Point2CAD: Reverse Engineering CAD Models from 3D Point Clouds

Computer-Aided Design (CAD) model reconstruction from point clouds is an important problem at the intersection of computer vision, graphics, and machine learning; it saves the designer significant time when iterating on in-the-wild objects. Recent advancements in this direction achieve relatively reliable semantic segmentation but still struggle to produce an adequate topology of the CAD model. In this work, we analyze the current state of the art for that ill-posed task and identify shortcomings of existing methods. We propose a hybrid analytic-neural reconstruction scheme that bridges the gap between segmented point clouds and structured CAD models and can be readily combined with different segmentation backbones. Moreover, to power the surface fitting stage, we propose a novel implicit neural representation of freeform surfaces, driving up the performance of our overall CAD reconstruction scheme. We extensively evaluate our method on the popular ABC benchmark of CAD models and set a new state-of-the-art for that dataset. Project page: https://www.obukhov.ai/point2cad}{https://www.obukhov.ai/point2cad.

==> figs/fig_inr_discussion.tex <==
\begin{figure}[t]
\begin{center}
   \includegraphics[width=1.0\linewidth]{imgs/inr_discussion}
\end{center}
    \caption{
    Visualization of noise resilience (\textbf{left}) and imperfect local minima (\textbf{right}) surface fitting with the proposed INR. 
    Overall, INR maintains the desired smoothness properties even in the presence of severe sample noise or convergence to local minima.
    Cf. Fig.~\ref{fig:inr:good} for the setting, legend, and color coding. 
    }
\label{fig:inr:discussion}
\end{figure}

==> figs/fig_noise_ablation.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth,trim={0 4em 0 0},clip]{imgs/noise_ablation.png}
% \includegraphics[width=\linewidth]{imgs/noise_ablation.png}
\caption{INR surface fitting without and with noise.}
\label{fig:inr_noise}
% \vspace{-18pt}
\end{figure}

==> figs/fig_samples.tex <==
\begin{figure*}[t!]
\centering
\includegraphics[width=0.95\linewidth]{imgs/samples.png}
\caption{Selected reconstructions with INR surfaces.}
\label{fig:samples}
\end{figure*}

==> tabs/tab_corners.tex <==
\begin{table*}[h]
\centering
\caption{Evaluation for \textit{Corners} after CAD Reconstruction}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
& & \multicolumn{3}{c}{$\theta_{\text{corner}}=0.03$} & \multicolumn{3}{c}{$\theta_{\text{corner}}=0.02$} & \multicolumn{3}{c}{$\theta_{\text{corner}}=0.01$}  \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
Method & Seg & precision~$\uparrow$ & recall~$\uparrow$ & F-score~$\uparrow$ & precision~$\uparrow$ & recall~$\uparrow$ & F-score~$\uparrow$ & precision~$\uparrow$ & recall~$\uparrow$ & F-score~$\uparrow$ \\
\midrule
ComplexGen & N/A & $0.667$ & $0.633$ & $0.650$ & $0.483$ & $0.454$ & $0.468$ & $0.217$ & $0.203$ & $0.210$ \\
Point2CAD & ParseNet & $\mathbf{0.669}$ & $\mathbf{0.634}$ & $\mathbf{0.651}$ & $\mathbf{0.494}$ & $\mathbf{0.547}$ & $\mathbf{0.519}$ & $0.349$ & $\mathbf{0.401}$ & $\mathbf{0.373}$ \\
Point2CAD & HPNet & $0.629$ & $0.620$ & $0.625$ & $0.476$ & $0.530$ & $0.502$ & $\mathbf{0.353}$ & $0.380$ & $0.366$\\
\midrule
Point2CAD & GT & $\underline{0.739}$ & $\underline{0.707}$ & $\underline{0.723}$ & $\underline{0.653}$ & $\underline{0.631}$ & $\underline{0.642}$ & $\underline{0.451}$ & $\underline{0.524}$ & $\underline{0.485}$\\
\bottomrule
\end{tabular}
} % \resizebox{\linewidth}{!}{
\label{tab:corner}
\end{table*}

==> tabs/tab_curves.tex <==
\begin{table*}[h]
\centering
\caption{Evaluation for \textit{Edges} after CAD Reconstruction}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
& & \multicolumn{3}{c}{$\theta_{\text{edge}}=0.06$} & \multicolumn{3}{c}{$\theta_{\text{edge}}=0.03$} & \multicolumn{3}{c}{$\theta_{\text{edge}}=0.02$}  \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
Method & Seg & precision~$\uparrow$ & recall~$\uparrow$ & F-score~$\uparrow$ & precision~$\uparrow$ & recall~$\uparrow$ & F-score~$\uparrow$ & precision~$\uparrow$ & recall~$\uparrow$ & F-score~$\uparrow$ \\
\midrule
ComplexGen & N/A & $0.687$ & $0.641$ & $0.663$ & $0.421$ & $0.396$ & $0.408$ & $0.290$ & $0.279$ & $0.284$ \\
Point2CAD & ParseNet & $\mathbf{0.689}$ & $0.644$ & $0.666$ & $0.426$ & $\mathbf{0.460}$ & $\mathbf{0.443}$ & $0.332$ & $\mathbf{0.381}$ & $0.355$ \\
Point2CAD & HPNet & $0.689$ & $0.645$ & $\mathbf{0.667}$ & $\mathbf{0.430}$ & $0.454$ & $0.442$ & $\mathbf{0.351}$ & $0.368$ & $\mathbf{0.360}$ \\
\midrule
Point2CAD & GT & $\underline{0.759}$ & $\underline{0.780}$ & $\underline{0.769}$ & $\underline{0.570}$ & $\underline{0.612}$ & $\underline{0.590}$ & $\underline{0.493}$ & $\underline{0.517}$ & $\underline{0.505}$\\
\bottomrule
\end{tabular}
} % \resizebox{\linewidth}{!}{
\label{tab:curve}
\end{table*}

==> tabs/tab_patches.tex <==
\begin{table*}[t]
\centering
\caption{Evaluation for \textit{Surfaces} after CAD Reconstruction}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
& & \multicolumn{3}{c}{$\theta_{\text{surface}}=0.08$} & \multicolumn{3}{c}{$\theta_{\text{surface}}=0.06$} & \multicolumn{3}{c}{$\theta_{\text{surface}}=0.03$}  \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
Method & Seg &precision~$\uparrow$ & recall~$\uparrow$ & F-score~$\uparrow$ & precision~$\uparrow$ & recall~$\uparrow$ & F-score~$\uparrow$ & precision~$\uparrow$ & recall~$\uparrow$ & F-score~$\uparrow$ \\
\midrule
ComplexGen & N/A & $0.732$ & $0.732$ & $0.731$ & $0.633$ & $0.641$ & $0.637$ & $0.370$ & $0.388$ & $0.379$ \\
Point2CAD & ParseNet & $0.776$ & $\mathbf{0.734}$ & $0.754$ & $0.720$ & $0.653$ & $0.685$ & $0.578$ & $0.520$ & $0.547$ \\
Point2CAD & HPnet & $\mathbf{0.815}$ & $0.733$ & $\mathbf{0.772}$ & $\mathbf{0.770}$ & $\mathbf{0.664}$ & $\mathbf{0.713}$ & $\mathbf{0.644}$ & $\mathbf{0.540}$ & $\mathbf{0.587}$\\
\midrule
Point2CAD & GT &$\underline{0.975}$ & $\underline{0.882}$ & $\underline{0.926}$ & $\underline{0.954}$ & $\underline{0.848}$ & $\underline{0.898}$ & $\underline{0.838}$ & $\underline{0.731}$ & $\underline{0.781}$\\
\bottomrule
\end{tabular}
} % \resizebox{\linewidth}{!}{
\label{tab:patch}
\end{table*}

